A Simple Analytic Treatment of Neutrino Mass Impact on the Full Power Spectrum Shape via a Two-Fluid Approximation

We present a new closed-form formula for the matter power spectrum in the presence of massive neutrinos that gives an accuracy of better than 5\% on all scales. It is the first closed-form result valid on all scales. To calculate this closed-form solution, we iteratively solve the fluid equations for cold dark matter+baryons, and neutrinos in terms of the neutrino mass fraction, $f_{\nu} \ll 1$, using variation of parameters to construct the response of the matter to the neutrino perturbation, which in turn will source the higher-order neutrino perturbations. This analytic solution accelerates calculations of the matter power spectrum with neutrinos. Also, it enables one to calculate the cross power spectra of matter and neutrinos which in turn can be used in computing the higher-order corrections to the power spectrum. To demonstrate our formula's accuracy and utility, we perform a Fisher forecast with it and show we reproduce the forecast from the Boltzmann solver class.

==> name.tex <==
\section{Dark Energy Effects}
\label{Dark Energy Modifications}

Up to now, we have discussed how massive neutrinos impact the power spectrum, as a function of scale, in a matter-dominated Universe. However, our Universe is not entirely Einstein-de Sitter (EdS): dark energy (DE) became the Universe's dominant componente at $z_{\rm{eq}} \approx 0.37$. The consequences of dark-energy-domination are interesting to discuss since our treatment {\bf ZS: this is puzzling---you refer to our treatment of dark energy, but we have not yet seen this!} of dark energy is \textbf{ZS: our treatment cannot be close to a physical effect---treatment is a mathematical approach, whereas ISW is a physical effect in the real world} very close to the late-time Integrated Sachs Wolfe (ISW) effect in the CMB \cite{Sachs:1967er}.

Let us imagin a gravitational potential well with some arbitrary depth along the line of sight. As the photons enter the well, they gain energy, and as they leave the well, they lose it. If the potential well does not change as they traverse it, the photons' net energy gain is zero (exactly what happens in an Einstein-de Sitter universe). However, when DE dominates, the potential changes as the Universe expands; therefore the photons will experience gravitational redshift. This effect corresponds to the picture we discussed earlier {\bf zS: where di we discuss this? tell the reader what section and what part} where the gravitational potential $\phi(k,\tau)$ enters (\ref{dcb})-(\ref{tnu}). Since in the DE-dominated Universe, the potential is not constant, its rate of change will affect the clustering of matter and of neutrinos on all scales. 

W incorporate DE in our fluid equations as follows. First, we focus on small scales {\bf ZS: small relative to what?} since these are the scales on which neutrinos leave their imprint. For these scales, the effect of the time-varying gravitational potential will be eliminated since it is coupled to the matter perturbations via the Poisson equation (\ref{Poisson}) and hence suppressed by a factor of $1/k^2$. We can rewrite the time derivative of the potential as:
% \begin{align}
%     \frac{-3\dot{\phi}}{\dot{\dnu}}\approx -3\frac{3}{2}\frac{\Omega_{{\rm m},0} \mathcal{H}_0^2}{k_0^2}\frac{(\dcb(k,\tau)/a)'}{(\dcb(k,\tau )a)'}\approx\frac{3}{2}\Omega_{{\rm m},0} \frac{\mathcal{H}_0^2}{k_0^2}\approx \left(\frac{\text{Free-Streaming Scale}}{\text{Horizon Size}}\right)^2\ll 1.
% \end{align}
\begin{align}
    \phi(k, a) = \frac{3}{2}\Omega_{\rm m}\left(\frac{a_0^2 H_0^2}{k^2}\right)\left(\frac{\delta}{a}\right) \propto \left(\frac{\text{Scales of Interest}}{\text{Horizon Size}}\right)^2
\end{align}
Since the scales of interest are smaller than the free-streaming scale of neutrinos, we can neglect the effects of the gravitational potential's evolution. 
{\bf ZS: ok, what do we do once we neglect that?}
{\bf ZS: this section is not really structured with any guiding words---like, you don't start by telling uus what we are going to try to do.}

Second, we implement the iterative method we discussed earlier. While we ignore the evolution of $\phi$, The DE changes the rate at which the universe is expanding. We perturbatively expand in $\fnu$ and order by order, solve the fluid equations. The system of equations we need to solve is exactly that of (\ref{dcb''}) and (\ref{dnu''}) but  with 
\begin{align}
    \frac{\mathcal{H}'}{\mathcal{H}}+1 = 2- \frac{3}{2}\left(\frac{1}{1+\Omega_{\Lambda}/\Omega_{\rm m}a^3}\right)= 2-\frac{3}{2}\left(\frac{1}{1+e^{3(s-s_{\rm{eq}})}}\right),
    \label{H}
\end{align}
where $s_{\rm{eq}}$ is the value of $s$ at matter-dark energy equality. As we can see, at early times, before equality, $s\ll s_{\rm{eq}}$ and therefore (\ref{H}) converges to $1/2$, recovering the matter-dominated solutions. The growing solution of the zeroth order CDM+baryon equation (\ref{dcb''}) then takes the form:
\begin{align}
    \dcb^{0}(q,s) = \mathcal{C}\,\dcb(k,s)\, \fone\left(\frac{1}{3},1,\frac{11}{6},-e^{3\left(s-s_{\rm{eq}}\right)}\right)
    \label{lambda matter solution}
\end{align}
where $\mathcal{C}$ is a normalization factor, $\dcb(k,s)$ is the present-time matter perturbation in an EdS Universe and $\fone$ is Gauss hypergeometric function. (\ref{lambda matter solution}) is consistent with earlier works on the effect of dark energy on the growth of matter perturbations such as \cite{linder2003cosmic}. 


\begin{figure}%
    \centering
    \subfloat{\includegraphics[width=12cm]{deltamatter0growth.pdf} }%
    \caption{The matter growth function vs. scale factor for two different cosmologies with $\Omega_{\Lambda} = 0$ and $\Omega_{\Lambda} = 0.7$ to show the suppression of growth in the presence of dark energy.}%
    \label{deltagrowth}%
\end{figure}

Fig. \ref{deltagrowth} shows how dark-energy domination changes the growth of the matter perturbations. It essentially suppresses the growth factor by almost $20\%$ at the present time. From the previous section it is clear that on small scales, the neutrinos are almost unperturbed. Therefore, we are safe to assume that on these scales $\dnu(q\rightarrow\infty,s) \approx 0$. 
The solution scheme in this case, as is generic for a second-order differential equation, is:
\begin{align}
    \dcb^{(1)}(q,s) = G(s)\left(c_1+Y_{{\rm P},G}\right)+D(s)\left(c_2+Y_{{\rm P},D}\right).
\end{align}
$G(s)$ is the growing mode and $D(s)$ the decaying mode of the homogeneous equation, $c_1$ and $c_2$ are constants, and $Y_{{\rm P},G}$ and $Y_{{\rm P},D}$ are the particular solutions of the non-homogeneous differential equation with a driving force of the form (\ref{lambda matter solution}). At the end, we need to eliminate the decaying mode since at early times it diverges. Therefore, we tune $c_2$ to remove it. This is only possible in a Universe where DE has taken over the expansion relatively recently. If $s_{\rm{eq}}$ is large enough, we cannot perform this tuning since the particular solution will not be close enough to a constant.

Therefore, the matter perturbation up to first order becomes:
\begin{align}
    \dm(q,s)&=\mathcal{C}\,\dcb(q,0)e^s\, \fone\left(\frac{1}{3},1,\frac{11}{6},-e^{3\left(s-s_{\rm{eq}}\right)}\right)
    \label{first order matter pt}\\&\times\left(1-\fnu+ \fnu \frac{\Gamma \left(\frac{11}{6}\right) \left[G_{3,3}^{2,2}\left(e^{3 s-3s_{\rm{eq}}} \bigg|
\begin{array}{c}
 0,\frac{2}{3},1 \\
 0,0,-\frac{5}{6} \\
\end{array}
\right)-G_{3,3}^{2,2}\left(e^{3s_{\rm T}-3 s_{\rm{eq}}} \bigg|
\begin{array}{c}
 0,\frac{2}{3},1 \\
 0,0,-\frac{5}{6} \\
\end{array}
\right)\right]}{5\Gamma \left(\frac{1}{3}\right)}\right),\nonumber
\end{align}
where $G_{3,3}^{2,2}$, is the Meijer $G$-function. One important consistency check is to verify that (\ref{first order matter pt}) converges to (\ref{dm}) when $s_{\rm{eq}}\rightarrow0$. In this limit, the two solutions do become the same up to zeroth order in $1/q^2$. With the consistency check passed, we find the power spectrum suppression as:
\begin{align}
    \frac{\delta P}{P_{\fnu=0}}=-2\fnu\Bigg(1+\frac{\Gamma \left(\frac{11}{6}\right) \left[G_{3,3}^{2,2}\left(e^{3 s-3s_{\rm{eq}}}\bigg|
\begin{array}{c}
 0,\frac{2}{3},1 \\
 0,0,-\frac{5}{6} \\
\end{array}
\right)-G_{3,3}^{2,2}\left(e^{3s_{\rm T}-3 s_{\rm{eq}}} \bigg|
\begin{array}{c}
 0,\frac{2}{3},1 \\
 0,0,-\frac{5}{6} \\
\end{array}
\right)\right]}{5\Gamma \left(\frac{1}{3}\right)}\Bigg).
\label{DEPSsupression}
\end{align}
